Conceptualization of seeded region growing by pixels aggregation. Part 3: a wide range of algorithms

In the two previous papers of this serie, we have created a library, called Population, dedicated to seeded region growing by pixels aggregation and we have proposed different growing processes to get a partition with or without a boundary region to divide the other regions or to get a partition invariant about the seeded region initialisation order. Using this work, we implement some algorithms belonging to the field of SRGPA using this library and these growing processes.

==> section4.tex <==
\section{swap queues}
